Classification Matters: Improving Video Action Detection with Class-Specific Attention

Video action detection (VAD) aims to detect actors and classify their actions in a video. We figure that VAD suffers more from classification rather than localization of actors. Hence, we analyze how prevailing methods form features for classification and find that they prioritize actor regions, yet often overlooking the essential contextual information necessary for accurate classification. Accordingly, we propose to reduce the bias toward actor and encourage paying attention to the context that is relevant to each action class. By assigning a class-dedicated query to each action class, our model can dynamically determine where to focus for effective classification. The proposed model demonstrates superior performance on three challenging benchmarks with significantly fewer parameters and less computation.

==> figures/04_method/LDL.tex <==
\begin{figure}
     \centering\
     \includegraphics[width=0.47\textwidth]{figures/04_method/LDL_simple3.pdf}
     \caption{Structure of Localizing Decoder Layer.}
     \label{Localizer}
     \vspace{-2mm}
\end{figure}

==> figures/04_method/location_biased_detections.tex <==
\begin{figure}
     \centering
     \includegraphics[width=\textwidth]{./figures/03_background/location_biased_detections.pdf}
     % \vspace{-6mm}
     \caption{
     Sample detection results and classification attention maps of the previous transformer-based model, TubeR~\cite{zhao2022tuber}, and our model.
     Each attention map signifies the regions where the model has attended to classify the action of the actor marked in the bounding box of the same color.
     Since our model creates an attention map for each label, we mark the corresponding label under the map.
     Although the GT label requires the model to pay attention to specific regions (``talk to (e.g., self, a person, a group)'', ``carry/hold (an object)'', and ``answer phone'') or even beyond the actor's location (``listen to (a person)''), the model's attention is primarily concentrated along the edge portion of the actor in TubeR. This behavior of the model can be interpreted as an attempt to classify the actor's pose specifically, but it ultimately results in the model overlooking other types of labels.
     On the other hand, our model seeks informative regions depending on the label, which assists model in carrying essential information for classification. Best viewed in color.}
     \label{location_biased_detections}
     \vspace{-4mm}
\end{figure}


==> figures/05_experiments/query_sa.tex <==
% \begin{figure}[htb]
%     \begin{minipage}[b]{0.50\textwidth}
%         \centering
%         \footnotesize
%         \begin{tabular}{lc}
%             \toprule
%             Method & AVA \\ 
%             \hline
%             w/ class query SA & 28.0 \\
%             w/o class query SA & 26.2 \\
%             \bottomrule
%         \end{tabular}
%         \vspace{1.2em}
%         \captionof{table}{Ablation experiments on the class query self-attention.}
%         \label{query_sa}
%     \end{minipage}%
%     \hspace{0.9em}
%     \begin{minipage}[b]{0.5\textwidth}
%         \centering
%         \subfloat[][]{\includegraphics[scale=0.1219]{figures/05_experiments/cqsa_1.png}\label{abl2:fig1}}
%         \hspace{0.005em}
%         \subfloat[][]{\includegraphics[scale=0.163]{figures/05_experiments/cqsa_2.png}\label{abl2:fig2}}
%         % \caption{\protect\subref{abl2:fig1} Class co-occurrence map of AVA v2.2  and \protect\subref{abl2:fig2} the self-attention map of the class queries.}
%         \caption{(a) Class co-occurrence map of AVA v2.2 and (b) self-attention map of the class queries.}        
%         % \caption{\ref{abl2:fig1} Class co-occurrence map of AVA v2.2 and \ref{abl2:fig2} the self-attention map of the class queries.}
%         \label{fig:selfattmap}
%     \end{minipage}
% \end{figure}
\begin{figure}
    \centering
    \subfloat[][]{\includegraphics[scale=0.15]{figures/05_experiments/cqsa_1.png}\label{abl2:fig1}}
    \hspace{4mm}
    \subfloat[][]{\includegraphics[scale=0.20]{figures/05_experiments/cqsa_2.png}\label{abl2:fig2}}
    % \caption{\protect\subref{abl2:fig1} Class co-occurrence map of AVA v2.2  and \protect\subref{abl2:fig2} the self-attention map of the class queries.}
    \caption{(a) Class co-occurrence map of AVA v2.2 and (b) self-attention map of the class queries.}        
    % \caption{\ref{abl2:fig1} Class co-occurrence map of AVA v2.2 and \ref{abl2:fig2} the self-attention map of the class queries.}
    \label{fig:selfattmap}
\end{figure}

==> figures/05_experiments/wopq.tex <==
\begin{figure}
     % \vspace{-10mm}
     \centering
     \includegraphics[width=0.5\textwidth]{figures/05_experiments/wopq_ver2-compressed.pdf}
     \caption{Visualizations on attaching the actor positional queries to the class queries.
     The following attention maps are from the class ``sit,'' and each map signifies the attended region that are employed to recognize the action of the actor marked with the bounding box.
     (a) shows the case where the positional queries are not appended to the class queries. Although the class ``sit'' does not require the model to observe areas beyond the actor location, they often activate regions where a similar actor performs the same action. 
     On the other hand, (b) shows the case where the positional queries are attached, and here the class queries are clearly aware of which actor they need to identify.}
     \label{wopq}
\end{figure}
 % which requires the model's ability to recognize the actor's specific pose
 % but not modulated. Modulated query design of DAB-DETR~\cite{liu2022dab} offers the model more accurate clues, especially when identifying the actor's precise height or width is important for classification. (c) illustrates the case of the current model, wherein the modulated query design is incorporated into the class queries.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> tables/CDL.tex <==
\begin{table}[!h]
\centering
% \vspace{5mm}
\caption{
Ablation experiments on classifying decoder layer (CDL).
}
\begin{tabular}{lcc}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{mAP} & when GT box \\ 
     &  & is provided \\ [0.2em]
\hline
\\[-1em]
    w/ CDL & 28.0 & $31.5_{(+3.5)}$ \\
    w/o CDL & 27.3 & $29.0_{(+1.7)}$ \\
    \bottomrule
\end{tabular}
\label{CDL}
% \vspace{-5mm}
\end{table}
% \vspace{5mm}


==> tables/actor_context_combine.tex <==
\begin{table}[t]
\centering
% \footnotesize
\begin{tabular}{lc}
\toprule
% {Method}  & AVA & UCF\\ 
% \hline
% \\[-1em]
% summation & 28.0 & - \\
% concat + 1d conv & 27.0 & - \\
% cross attention & 26.7 & - \\

{Method}  & AVA \\ 
\hline
\\[-1em]
summation & 28.0 \\
concat + 1d conv & 27.0 \\
cross-attention & 26.7 \\


\bottomrule
\end{tabular}
\caption{Ablation experiments on ways to combine the actor and context features.}
\label{actor_context_combine}
\end{table}

==> tables/actor_query_pos_and_msss.tex <==
\begin{figure}[htb]
    % \vspace{-2mm}
    \begin{minipage}[t]{0.45\textwidth}
        \centering
        \captionof{table}{Ablation experiments on utilizing multi-scale feature maps.}
        \vspace{1mm}
        \input{tables/multiscale_vs_singlescale}
        % \vspace{1.2em}
        % \vspace{-10mm}
    \end{minipage}
    \hspace{0.9em}
    \begin{minipage}[t]{0.5\textwidth}
    \centering
    \captionof{table}{The effect of attaching the actor positional queries to the class queries.}
    \vspace{1mm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcc}
        \toprule
        {Method}  & AVA & UCF \\ 
        \hline
        \\[-1em]
        % w/ modulated actor positional queries & 33.4 & 84.8 \\
        w/ actor positional queries & 33.4 & 84.8 \\
        % w/ ordinary actor positional queries & 32.7 & 84.8 \\
        w/o actor positional queries & 31.7 & 82.9 \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{-4mm}
    \label{actor_query_pos}
    \end{minipage}

\end{figure}

==> tables/classification_is_the_key.tex <==

\begin{table*}[t]
\centering
\begin{tabular}{lcccccc}
\toprule
{Model}                                         & Dataset                 & Backbone  & Pre-train     & {f-mAP@0.5} & {w/ GT box}           & {w/ GT class label} \\ 
\hline
\\[-1em]
\multirow{4}{*}{TubeR~\cite{zhao2022tuber}}     & \multirow{2}{*}{AVA2.1} & CSN-50    & K400          & {27.2}      & {30.6}$_{(+3.4)}$    & 91.9$_{(+64.7)}$              \\ 
                                                &                         & CSN-152   & IG+K400       & {29.7}      & {33.3}$_{(+3.6)}$    & 90.8$_{(+61.1)}$              \\ \cline{2-7} 
\\[-0.8em]
                                                & AVA2.2                  & CSN-152   & IG+K400       & {31.1}      & {34.2}$_{(+3.1)}$    & 93.3$_{(+62.2)}$              \\ \cline{2-7} 
\\[-0.8em]
                                                & JHMDB                   & CSN-152   & IG+K400       & {72.2}      & {74.9}$_{(+2.7)}$    & 77.5$_{(+5.3)}$              \\ 
\bottomrule
\end{tabular}
\caption{The spatio-temporal action detection result based on TubeR~\cite{zhao2022tuber}, given GT annotations. In the "w/ GT box" setting, we measure f-mAP at near-zero IoU, providing the model a very generous assumption of wherever the model localizes, there exists a desired target object. In the "w/ GT class label" setting, the incorrect label of the prediction is eliminated, regarding that the target object with IoU larger than the threshold is what the detection aimed to detect.}
\label{classification_is_the_key}
\end{table*}




==> tables/classification_metric.tex <==
\begin{table}[t]
\caption{Performance comparison on the latest VAD models. We have measured the classification ability of each model by replacing box prediction results to ground-truth (GT) box coordinates.}
\fontsize{7.8}{9.5}\selectfont
\centering
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{f-mAP} & when GT box \\ 
 &  &  & is provided \\ [0.2em]
\hline
\\[-1em]
TubeR & CSN-152 & 31.1 & $33.1_{(+2.0)}$ \\
STMixer & ViT-B & 32.6 & $34.7_{(+2.1)}$ \\
STMixer & ViT-B~\cite{wang2023videomae} & 36.1 & $38.7_{(+2.6)}$ \\
EVAD & ViT-B & 32.3 & $34.5_{(+2.2)}$ \\
EVAD & ViT-B~\cite{wang2023videomae} & 37.7 & $40.0_{(+2.3)}$ \\
\rowcolor{Gray!20}
Ours & CSN-152 & \textbf{33.5} & $\mathbf{37.2_{(+3.7)}}$ \\
\rowcolor{Gray!20}
Ours & ViT-B & \textbf{32.9} & $\mathbf{36.9_{(+4.0)}}$ \\
\rowcolor{Gray!20}
Ours & ViT-B~\cite{wang2023videomae} & \textbf{38.4} & $\mathbf{42.1_{(+3.7)}}$ \\


\bottomrule
\end{tabular}
\label{classification metric 2}
\end{table}

==> tables/decoder_depth.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lcccc}
\toprule
{Decoder depth}  & 1  & 3   & 6 & 9 \\ 
\hline
\\[-1em]
AVA & 26.4 & 27.5 & \textbf{28.0} & 25.6 \\
UCF & - & - & - & - \\

\bottomrule
\end{tabular}
\caption{Decoder depth}
\label{decoder_depth}
\end{table}

==> tables/encoder_depth.tex <==

\begin{table}[t]
\centering
\begin{tabular}{lccccc}
\toprule
{Encoder depth}           & 0                 & 1  & 3     & 6 & 9 \\ 
\hline
\\[-1em]
AVA & 25.6 & 26.7 & 27.5 & \textbf{28.0} & 27.1 \\
UCF & - & - & - & - & -\\

\bottomrule
\end{tabular}
\caption{Encoder depth}
\label{encoder_depth}
\end{table}



==> tables/flops.tex <==
% \newcommand{\quhqu}{ \ \ - \ \ }

\begin{table}[t]
\centering
\caption{FLOPs comparison on JHMDB51-21 and UCF101-24. We count the amount of computation needed to output a 40-frame tube for JHMDB51-21, and 32-frame tube for UCF, considering each RGB frame's resolution as 256 $\times$ 360.}
% \footnotesize
\vspace{-2mm}
\scalebox{0.75}{
\begin{tabular}{>{\raggedright\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{2.3cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{2.4cm}>{\centering\arraybackslash}m{3.8cm}}
\toprule
{Method} & {Backbone} & {Input $(T \times \tau)$ }         & {Params}  & {FLOPs}  & {\scriptsize Inf. time (ms)}  & {f-mAP/v-mAP}  \\ 
\hline
\\[-1em]
\multicolumn{7}{l}{\textbf{JHMDB}: inferring a 40-frame tube}\\
\hline
\\[-1em]
TubeR    & CSN-152  & $32 \times 2$ & 91.8M   & 6.99T  & 1263.1  & \quhqu / \undreline{82.3} \\
STMixer  & SF-R101-NL & $32 \times 2$ & 219.2M   & 7.64T  & 2088.2  & 86.7 / \quhqu \\
EVAD     & ViT-B    & $16 \times 4$ & 185.4M  & 10.68T & 8363.1 & \textbf{90.2} / 77.8 \\
\rowcolor{Gray!20}
% Ours     & CSN-152  & $40 \times 1$ & 79.1M   & \textbf{3.99T}    & xx.x / xx.x \\
% \rowcolor{Gray!20}
% Ours     & ViT-B    & $40 \times 1$ & 117.8M  & \textbf{4.32T}    & xx.x / xx.x \\
% Ours     & ViT-B    & $40 \times 1$ & 104.0M  & \textbf{2.82T}    & 79.0 / 82.7 \\
% \rowcolor{Gray!20}
% Ours     & ViT-B    & $40 \times 1$ & 104.0M  & \textbf{2.82T}    & \fixed{79.9 / 83.3} \\
% \hline
Ours     & ViT-B    & $40 \times 1$ & 117.8M  & \textbf{3.26T}  & \textbf{432.0}  & {\underline{86.9}} / \textbf{90.0} \\
\hline
\\[-1em]
\multicolumn{7}{l}{\textbf{UCF}: inferring a 32-frame tube}\\
\hline
\\[-1em]
TubeR    & CSN-152  & $32 \times 2$ & 91.8M   & 5.60T  & 1161.9 & 83.2 / 58.4 \\
STMixer  & SF-R101-NL & $32 \times 2$ & 219.2M  & 6.12T  & 1671.5 & 83.7 / \quhqu \\
EVAD     & ViT-B    & $16 \times 4$ & 185.4M  & 8.54T  & 6797.8 & \textbf{85.1} / \underline{58.8} \\
\rowcolor{Gray!20}
% Ours     & CSN-152  & $32 \times 1$ & 86.0M   & \textbf{3.81T}    & xx.x / xx.x \\
% \rowcolor{Gray!20}
% Ours     & ViT-B    & $32 \times 1$ & 138.5M  & \textbf{5.55T}    & xx.x / xx.x \\
Ours     & ViT-B    & $32 \times 1$ & 117.8M  & \textbf{3.73T}  & \textbf{370.0}  & \underline{84.8} / \textbf{63.2} \\

\bottomrule
\end{tabular}
}
\label{flops}
\end{table}

==> tables/flops_and_classification_metric_backup.tex <==
\begin{figure}[t!]
    % \captionsetup{font=scriptsize}
    \vspace{-2mm}
    \begin{minipage}[t]{0.56\textwidth}
    \centering
    \captionof{table}{Efficiency comparison on JHMDB and UCF. Each frame's resolution is set to 256 $\times$ 360.
    % Single NVIDIA A100 GPU is used for inference.
    }
    \vspace{1mm}
        \scalebox{0.62}{
        \begin{tabular}{>{\raggedright\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{2.3cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{2.4cm}>{\centering\arraybackslash}m{3.8cm}}
        \toprule
        {Method} & {Backbone} & {Input $(T \times \tau)$ }         & {Params}  & {FLOPs}  & {\scriptsize Inf. time (ms)}  & {f-mAP/v-mAP}  \\ 
        \hline
        \\[-1em]
        \multicolumn{7}{l}{\textbf{JHMDB}: inferring a 40-frame tube}\\
        \hline
        \\[-1em]
        TubeR    & CSN-152  & $32 \times 2$ & \textbf{91.8M}   & 6.99T  & 1263.1  & \quhqu / \underline{82.3} \\
        STMixer  & SF-R101-NL & $32 \times 2$ & 219.2M   & 7.64T  & 2088.2  & 86.7 / \quhqu \\
        EVAD     & ViT-B    & $16 \times 4$ & 185.4M  & 10.68T & 8363.1 & \textbf{90.2} / 77.8 \\
        \rowcolor{Gray!20}
        % Ours     & CSN-152  & $40 \times 1$ & 79.1M   & \textbf{3.99T}    & xx.x / xx.x \\
        % \rowcolor{Gray!20}
        % Ours     & ViT-B    & $40 \times 1$ & 117.8M  & \textbf{4.32T}    & xx.x / xx.x \\
        % Ours     & ViT-B    & $40 \times 1$ & 104.0M  & \textbf{2.82T}    & 79.0 / 82.7 \\
        % \rowcolor{Gray!20}
        % Ours     & ViT-B    & $40 \times 1$ & 104.0M  & \textbf{2.82T}    & \fixed{79.9 / 83.3} \\
        % \hline
        Ours     & ViT-B    & $40 \times 1$ & \underline{117.8M}  & \textbf{3.26T}  & \textbf{432.0}  & {\underline{86.9}} / \textbf{88.5} \\
        \hline
        \\[-1em]
        \multicolumn{7}{l}{\textbf{UCF}: inferring a 32-frame tube}\\
        \hline
        \\[-1em]
        TubeR    & CSN-152  & $32 \times 2$ & \textbf{91.8M}   & 5.60T  & 1161.9 & 83.2 / 58.4 \\
        STMixer  & SF-R101-NL & $32 \times 2$ & 219.2M  & 6.12T  & 1671.5 & 83.7 / \quhqu \\
        EVAD     & ViT-B    & $16 \times 4$ & 185.4M  & 8.54T  & 6797.8 & \underline{85.1} / \underline{58.8} \\
        \rowcolor{Gray!20}
        % Ours     & CSN-152  & $32 \times 1$ & 86.0M   & \textbf{3.81T}    & xx.x / xx.x \\
        % \rowcolor{Gray!20}
        % Ours     & ViT-B    & $32 \times 1$ & 138.5M  & \textbf{5.55T}    & xx.x / xx.x \\
        Ours     & ViT-B    & $32 \times 1$ & \underline{117.8M}  & \textbf{3.73T}  & \textbf{370.0}  & \textbf{85.9} / \textbf{61.7} \\        
        % Ours     & ViT-B    & $32 \times 1$ & \underline{117.8M}  & \textbf{3.73T}  & \textbf{370.0}  & \underline{85.0} / \textbf{62.7} \\
        
        \bottomrule
        \end{tabular}
        }
        \label{flops}
    % \vspace{5mm}
    \end{minipage}
    \hspace{0.9em}
    \begin{minipage}[t]{0.4\textwidth}
        \centering
        \captionof{table}{Performance comparison on the latest VAD models.}
        \vspace{1mm}
        \scalebox{0.755}{
        \begin{tabular}{lccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{f-mAP} & when GT box \\ 
         &  &  & is provided \\ [0.2em]
        \hline
        \\[-1em]
        TubeR & CSN-152 & 31.1 & $33.1_{(+2.0)}$ \\
        STMixer & ViT-B & 32.6 & $34.7_{(+2.1)}$ \\
        STMixer & ViT-B~\cite{wang2023videomae} & 36.1 & $38.7_{(+2.6)}$ \\
        EVAD & ViT-B & 32.3 & $34.5_{(+2.2)}$ \\
        EVAD & ViT-B~\cite{wang2023videomae} & 37.7 & $40.0_{(+2.3)}$ \\
        \rowcolor{Gray!20}
        Ours & CSN-152 & \textbf{33.5} & $\mathbf{37.2_{(+3.7)}}$ \\
        \rowcolor{Gray!20}
        Ours & ViT-B & \textbf{32.9} & $\mathbf{36.9_{(+4.0)}}$ \\
        \rowcolor{Gray!20}
        Ours & ViT-B~\cite{wang2023videomae} & \textbf{38.4} & $\mathbf{42.1_{(+3.7)}}$ \\

        \bottomrule
        \end{tabular}
        }
        \label{classification metric 2}
        % \vspace{1.2em}
    \end{minipage}
    \vspace{-2mm}
\end{figure}

==> tables/flops_and_classification_metric_with_Na.tex <==
\setlength{\floatsep}{0pt plus 0pt minus 10pt}
\setlength{\textfloatsep}{12pt plus 0pt minus 5pt}
\begin{figure}[t!]
    % \captionsetup{font=scriptsize}
    \begin{minipage}[t]{0.61\textwidth}
    \centering
    \captionof{table}{Efficiency comparison on JHMDB and UCF. Each frame's resolution is set to 256 $\times$ 360.
    % Single NVIDIA A100 GPU is used for inference.
    }
        \scalebox{0.59}{
        \begin{tabular}{>{\raggedright\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{2.3cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{0.8cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{2.4cm}>{\centering\arraybackslash}m{3.8cm}}
        \toprule
        {Method} & {Backbone} & {Input $(T \times \tau)$ }    & $N_a$     & {Params}  & {FLOPs}  & {\scriptsize Inf. time (ms)}  & {f-mAP/v-mAP}  \\ 
        \hline
        \\[-1em]
        \multicolumn{7}{l}{\textbf{JHMDB}: inferring a 40-frame tube}\\
        \hline
        \\[-1em]
        TubeR    & CSN-152  & $32 \times 2$ & 15 & \textbf{91.8M}   & 6.99T  & 1263.1  & \:\:-\:\: / \underline{82.3} \\
        STMixer  & SF-R101-NL & $32 \times 2$ & 100 & 219.2M   & 7.64T  & 2088.2  & 86.7 / \:\:-\:\: \\
        EVAD     & ViT-B    & $16 \times 4$ & 100 & 185.4M  & 10.68T & 8363.1 & \textbf{90.2} / 77.8 \\
        \rowcolor{Gray!20}
        % Ours     & CSN-152  & $40 \times 1$ & 79.1M   & \textbf{3.99T}    & xx.x / xx.x \\
        % \rowcolor{Gray!20}
        % Ours     & ViT-B    & $40 \times 1$ & 117.8M  & \textbf{4.32T}    & xx.x / xx.x \\
        % Ours     & ViT-B    & $40 \times 1$ & 104.0M  & \textbf{2.82T}    & 79.0 / 82.7 \\
        % \rowcolor{Gray!20}
        % Ours     & ViT-B    & $40 \times 1$ & 104.0M  & \textbf{2.82T}    & \fixed{79.9 / 83.3} \\
        % \hline
        Ours     & ViT-B    & $40 \times 1$ & 5 & \underline{117.8M}  & \textbf{3.26T}  & \textbf{432.0}  & {\underline{86.9}} / \textbf{88.5} \\
        \hline
        \\[-1em]
        \multicolumn{7}{l}{\textbf{UCF}: inferring a 32-frame tube}\\
        \hline
        \\[-1em]
        TubeR    & CSN-152  & $32 \times 2$ & 15 & \textbf{91.8M}   & 5.60T  & 1161.9 & 83.2 / 58.4 \\
        STMixer  & SF-R101-NL & $32 \times 2$ & 100 & 219.2M  & 6.12T  & 1671.5 & 83.7 / \:\:-\:\: \\
        EVAD     & ViT-B    & $16 \times 4$ & 100 & 185.4M  & 8.54T  & 6797.8 & \underline{85.1} / \underline{58.8} \\
        \rowcolor{Gray!20}
        % Ours     & CSN-152  & $32 \times 1$ & 86.0M   & \textbf{3.81T}    & xx.x / xx.x \\
        % \rowcolor{Gray!20}
        % Ours     & ViT-B    & $32 \times 1$ & 138.5M  & \textbf{5.55T}    & xx.x / xx.x \\
        Ours     & ViT-B    & $32 \times 1$ & 15 & \underline{117.8M}  & \textbf{3.73T}  & \textbf{370.0}  & \textbf{85.9} / \textbf{61.7} \\        
        % Ours     & ViT-B    & $32 \times 1$ & \underline{117.8M}  & \textbf{3.73T}  & \textbf{370.0}  & \underline{85.0} / \textbf{62.7} \\
        
        \bottomrule
        \end{tabular}
        }
        \label{flops}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.37\textwidth}
        \centering
        \captionof{table}{Performance comparison on the latest VAD models.}
        \scalebox{0.72}{
        \begin{tabular}{lccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{f-mAP} & when GT box \\ 
         &  &  & is provided \\ [0.2em]
        \hline
        \\[-1em]
        TubeR & CSN-152 & 31.1 & $33.1_{(+2.0)}$ \\
        STMixer & ViT-B & 32.6 & $34.7_{(+2.1)}$ \\
        STMixer & ViT-B~\cite{wang2023videomae} & 36.1 & $38.7_{(+2.6)}$ \\
        EVAD & ViT-B & 32.3 & $34.5_{(+2.2)}$ \\
        EVAD & ViT-B~\cite{wang2023videomae} & 37.7 & $40.0_{(+2.3)}$ \\
        \rowcolor{Gray!20}
        Ours & CSN-152 & \textbf{33.5} & $\mathbf{37.2_{(+3.7)}}$ \\
        \rowcolor{Gray!20}
        Ours & ViT-B & \textbf{32.9} & $\mathbf{36.9_{(+4.0)}}$ \\
        \rowcolor{Gray!20}
        Ours & ViT-B~\cite{wang2023videomae} & \textbf{38.4} & $\mathbf{42.1_{(+3.7)}}$ \\

        \bottomrule
        \end{tabular}
        }
        \label{classification metric 2}
    \end{minipage}
\end{figure}

==> tables/gt_replacement.tex <==
\begin{table}[htb]
\fontsize{7.8}{9.5}\selectfont
\centering
\vspace{-2mm}
\scalebox{0.92}{
\begin{tabular}{lcccc}
\toprule
{Method} & Backbone & mAP & when GT box & when GT class\\ 
\quad & \quad & \ & is provided & is provided\\ 
\hline
\\[-1em]
TubeR [43] & CSN-152 & $31.1$ & $33.1_{(+2.0)}$ & $85.1_{(+54.0)}$ \\
STMixer [42] & ViT-B & $32.6$ & $34.7_{(+2.1)}$ & $\mathbf{93.5_{(+60.9)}}$ \\
STMixer [42] & ViT-B [35] & $36.1$ & $38.7_{(+2.6)}$ & $\mathbf{98.9_{(+60.2)}}$ \\
% STMixer [42] & ViT-B [35] & $36.1$ & $38.7_{(+2.6)}$ & $TBD$ \\
EVAD [2] & ViT-B & 32.3 & $34.5_{(+2.2)}$ & $91.5_{(+59.2)}$ \\
EVAD [2] & ViT-B [35] & 37.7 & $40.0_{(+2.3)}$ & $92.8_{(+55.1)}$ \\
\rowcolor{Gray!20}
Ours & CSN-152 & $\mathbf{33.5}$ & $\mathbf{37.2_{(+3.7)}}$ & $\mathbf{91.5_{(+58.0)}}$ \\
\rowcolor{Gray!20}
Ours & ViT-B & $\mathbf{32.9}$ & $\mathbf{36.9_{(+4.0)}}$ & $87.8_{(+54.9)}$ \\
\rowcolor{Gray!20}
Ours & ViT-B [35] & $\mathbf{38.4}$ & $\mathbf{42.1_{(+3.7)}}$ & $92.5_{(+54.1)}$ \\


\bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{Performance comparison on VAD models when their box and class predictions are replaced with ground-truth (GT) labels.}
\vspace{-3mm}
\label{gt_replacement}
\end{table}

==> tables/main_table_filtered.tex <==
% \begin{table*}[t]
% \footnote
% \centering
\scalebox{.82}{
\begin{tabular}{lccccccc}
% \footnote
\toprule
Model                                        & \:\emph{D}\:                & Input        & Backbone      & Pre-train   & mAP \\ 
\hline
\\[-1em]
SlowFast~\cite{feichtenzofer2019slowfast}      &\cmark                   &  $32 \times 2$ & SF-R101-NL    & K600          & {29.0}  \\ 
ACAR~\cite{pan2021actor}                       &\cmark                   &  $32 \times 2$ & SF-R101-NL    & K600          & {31.4}  \\ 
AIA~\cite{tang2020asynchronous}                &\cmark                   &  $32 \times 2$ & SF-R101       & K700          & {32.3}  \\ 
VideoMAE~\cite{tong2022videomae}               &\cmark                   &  $16 \times 4$ & ViT-B         & K400          & {31.8}  \\ 
% MeMViT~\cite{wu2022memvit}                     &\cmark                   &  $16 \times 4$ & MViTv2-S      & K400          & {28.5}  \\ 
MeMViT~\cite{wu2022memvit}                     &\cmark                   &  $32 \times 3$ & MViTv2-B      & K600          & {32.8}  \\ 
WOO~\cite{chen2021watch}                       & \xmark                  &  $32 \times 2$ & SF-R101-NL    & K600          & {28.3}  \\ 
% WOO~\cite{chen2021watch}                       & \xmark                  &  $16 \times 4$ & ViT-B         & K400          & ${30.0}^{\ddag}$  \\ 
TubeR~\cite{zhao2022tuber}                     & \xmark                  &  $32 \times 2$ & CSN-152       & IG65M, K400   & {31.1}  \\ 
% STAR/B~\cite{gritsenko2023end}                 & \xmark                  &  $32 \times 2$ & ViT-B         & IN21K, K400   & {30.0}  \\ 
STMixer~\cite{wu2023stmixer}                   & \xmark                  &  $32 \times 2$ & CSN-152       & IG65M, K400   & \underline{32.8}  \\ 
STMixer~\cite{wu2023stmixer}                   & \xmark                  &  $16 \times 4$ & ViT-B         & K400          & \underline{32.6}  \\ 
STMixer~\cite{wu2023stmixer}                   & \xmark                  &  $16 \times 4$ & ViT-B~\cite{wang2023videomae}         & K710, K400    & {36.1}  \\
EVAD~\cite{chen2023efficient}                  & \xmark                  &  $16 \times 4$ & ViT-B         & K400          & {32.3}  \\
EVAD~\cite{chen2023efficient}                  & \xmark                  &  $16 \times 4$ & ViT-B~\cite{wang2023videomae}         & K710, K400    & \underline{37.7}  \\
% \hline
\rowcolor{Gray!20}
Ours                                           & \xmark                  &  $32 \times 2$ & CSN-152       & IG65M, K400   & {\textbf{33.5}}  \\ 
\rowcolor{Gray!20}
Ours                                           & \xmark                  &  $16 \times 4$ & ViT-B         & K400          & {\textbf{32.9}}  \\
\rowcolor{Gray!20}
Ours                                           & \xmark                  &  $16 \times 4$ & ViT-B~\cite{wang2023videomae}         & K710, K400    & {\textbf{38.4}} \\
% \rowcolor{Gray!20}
% Ours                                          & \xmark                  &  $32 \times 2$ & ViT-B         & K600          & {29.0}  \\ 

\bottomrule
\end{tabular}
}
% \caption{Main Table}
% \label{main_table}
% \end{table*}

==> tables/module_ablations_and_msss_and_cqsa_backup.tex <==
\begin{figure}[t!]
    % \captionsetup{font=scriptsize}
    % \vspace{-2mm}
    \begin{minipage}[t]{0.5\textwidth}
        \centering
        \captionof{table}{Ablation experiments on each module of the model.}
        \vspace{1mm}
        \scalebox{.85}{
        \begin{tabular}{llc}
            \toprule
            {Encoder} & {Decoder} & mAP \\ 
            \hline
            \\[-1em]
            Transformer & DETR & 28.6 \\ % 270-238
            Transformer & LDL & 29.1 \\ % 270-645
            Transformer & LDL + CDL & 31.4 \\
            % 3D Deformable Transformer \ & DETR & 24.4 \\ % 270-640
            3D Deformable Transformer \ & LDL & 31.3 \\
            3D Deformable Transformer \ & LDL + CDL & 33.5 \\
            \bottomrule
        \end{tabular}\label{abl:modules}
        }
        \vspace{-1mm}
        \setcounter{table}{2}
        \captionof{table}{Effect of attaching the actor positional queries to class queries.}
        \vspace{1.5mm}
        % \resizebox{\textwidth}{!}{
        \scalebox{.90}{
        \begin{tabular}{lcc}
            \toprule
            {Method}  & AVA & UCF \\ 
            \hline
            \\[-1em]
            % w/ modulated actor positional queries & 33.4 & 84.8 \\
            % w/ actor positional queries \qquad \qquad & 33.5 & 85.0 \\
            w/ actor positional queries \qquad \qquad & 33.5 & 85.9 \\
            % w/ ordinary actor positional queries & 32.7 & 84.8 \\
            w/o actor positional queries \qquad \qquad & 31.7 & 82.9 \\
            \bottomrule
        \end{tabular}\label{abl:positional_queries}
        }
    
        % \vspace{1.2em}
        % \vspace{-10mm}
    \end{minipage}
    \hspace{0.6em}
    \begin{minipage}[t]{0.45\textwidth}
    \centering
    \setcounter{table}{1}
    \captionof{table}{Ablation experiments on ways to aggregate multi-scale feature maps.}
    \vspace{1mm}
    \scalebox{.9}{
        \input{tables/multiscale_vs_singlescale}\label{abl:msss}
        }
    \vspace{-0.5mm}
    % \vspace{0.5mm}
    \setcounter{table}{3}
    \captionof{table}{Ablation experiments on ways to combine actor and context features.}
    \vspace{1mm}
    \scalebox{.87}{
        \begin{tabular}{lcc}
            \toprule
            {Method}  & AVA & UCF\\ 
            \hline
            \\[-1em]
            summation & 33.5 & 85.9 \\
            concat + 1d conv~\cite{sun2018actor} \qquad \qquad & 31.8 & 84.7 \\
            cross-attention~\cite{zhao2022tuber} & 31.3 & 81.3 \\
            self-attention~\cite{chen2023efficient} & 30.8 & 81.0 \\
            \bottomrule
        \end{tabular}\label{abl:comb_actor_context}
    }
    % \vspace{-4mm}
    \label{msss2}
    \end{minipage}

\end{figure}
